PixelGen: Rethinking Embedded Camera Systems

Embedded camera systems are ubiquitous, representing the most widely deployed example of a wireless embedded system. They capture a representation of the world - the surroundings illuminated by visible or infrared light. Despite their widespread usage, the architecture of embedded camera systems has remained unchanged, which leads to limitations. They visualize only a tiny portion of the world. Additionally, they are energy-intensive, leading to limited battery lifespan. We present PixelGen, which re-imagines embedded camera systems. Specifically, PixelGen combines sensors, transceivers, and low-resolution image and infrared vision sensors to capture a broader world representation. They are deliberately chosen for their simplicity, low bitrate, and power consumption, culminating in an energy-efficient platform. We show that despite the simplicity, the captured data can be processed using transformer-based image and language models to generate novel representations of the environment. For example, we demonstrate that it can allow the generation of high-definition images, while the camera utilises low-power, low-resolution monochrome cameras. Furthermore, the capabilities of PixelGen extend beyond traditional photography, enabling visualization of phenomena invisible to conventional cameras, such as sound waves. PixelGen can enable numerous novel applications, and we demonstrate that it enables unique visualization of the surroundings that are then projected on extended reality headsets. We believe, PixelGen goes beyond conventional cameras and opens new avenues for research and photography.

==> Sections/dummy_text.tex <==
%\begin{figure}
 %   \centering
 %   \includegraphics[width=\textwidth/2]{figures/himax.png} 
%    \caption{Monochrome Camera}
 %   \label{fig:Monochrome Cameral}
%\end{figure}



% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/example_day.png}
%     \caption{The image generated of resolution 972 x 732 based on positive prompt: overcast (lux = 1036), warm (temperature = 24.94), humid (percentage = 67.09), null(pressure = 100573), and the original image is preprocessed by Oneformer segmentation model.}
%     \label{fig:Example1}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \textbf{\hl{Ambuj: Can we show intermediate inputs here and show the final output eventually!! This will make the narrative quite clear.}}
% % \textbf{\hl{Kunjun: We can show 2-3 different scenarios here, with same monochrome image and vary one of the environmental parameters and show it's impact. Definitely, we need 5+ results here. We have to show their corresponding prompt, controlnet output and then final output. Have to discuss with Ambuj for the control flow of these images!!}}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/example_sunlight.png}
%     \caption{The image generated of resolution 972 x 732 based on positive prompt: bright sunlight (lux = 8407), hot (temperature = 29.52), humid (percentage = 63.11), null (pressure = 100687), and the original image is preprocessed by Canny Edge Detector.}
%     \label{fig:Example2}
% \end{figure}


